Model Counting in Product Configuration

We describe how to use propositional model counting for a quantitative analysis of product configuration data. Our approach computes valuable meta information such as the total number of valid configurations or the relative frequency of components. This information can be used to assess the severity of documentation errors or to measure documentation quality. As an application example we show how we apply these methods to product documentation formulas of the Mercedes-Benz line of vehicles. In order to process these large formulas we developed and implemented a new model counter for non-CNF formulas. Our model counter can process formulas, whose CNF representations could not be processed up till now.

==> eptcsdata.tex <==
\providecommand{\event}{I. Lynce and R. Treinen (eds.): Workshop on\\
Logics for Component Configuration (LoCoCo 2010)}
\providecommand{\volume}{29}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{44}
\providecommand{\eid}{5}
\providecommand{\publicationstatus}{I. Lynce and R. Treinen (eds.): Workshop on\\
Logics for Component Configuration (LoCoCo 2010)\\
EPTCS 29, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.29.5}{10.4204/EPTCS.29.5}}

